HEK VI: On the Dearth of Galilean Analogs in Kepler and the Exomoon Candidate Kepler-1625b I

Exomoons represent an outstanding challenge in modern astronomy, with the potential to provide rich insights into planet formation theory and habitability. In this work, we stack the phase-folded transits of 284 viable moon hosting Kepler planetary candidates, in order to search for satellites. These planets range from Earth-to-Jupiter sized and from ${\sim}$0.1-to-1.0 AU in separation - so-called "warm" planets. Our data processing includes two-pass harmonic detrending, transit timing variations, model selection and careful data quality vetting to produce a grand light curve with an r.m.s. of 5.1 ppm. We find that the occurrence rate of Galilean-analog moon systems for planets orbiting between ${\sim}$0.1 and 1.0 AU can be constrained to be $\eta<0.38$ to 95% confidence for the 284 KOIs considered, with a 68.3% confidence interval of $\eta=0.16_{-0.10}^{+0.13}$. A single-moon model of variable size and separation locates a slight preference for a population of short-period moons with radii ${\sim}0.5$ $R_{\oplus}$ orbiting at 5-10 planetary radii. However, we stress that the low Bayes factor of just 2 in this region means it should be treated as no more than a hint at this time. Splitting our data into various physically-motivated subsets reveals no strong signal. The dearth of Galilean-analogs around warm planets places the first strong constraint on exomoon formation models to date. Finally, we report evidence for an exomoon candidate Kepler-1625b I, which we briefly describe ahead of scheduled observations of the target with the Hubble Space Telescope.

==> journals.tex <==
\newcommand{\aj}{{\it AJ}}% UNCOMMENTED
          % Astronomical Journal
\newcommand{\actaa}{{\it Acta Astron.}}%
          % Acta Astronomica
%\newcommand{\araa}{{\it ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand{\apj}{{\it ApJ}}% UNCOMMENTED
          % Astrophysical Journal
\newcommand{\apjl}{{\it ApJ}}% UNCOMMENTED
          % Astrophysical Journal, Letters
%\newcommand{\apjs}{{\it ApJS}}%
          % Astrophysical Journal, Supplement
%\newcommand{\ao}{{\it Appl.~Opt.}}%
          % Applied Optics
%\newcommand{\apss}{{\it Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand{\aap}{{\it A\&A}}% UNCOMMENTED
          % Astronomy and Astrophysics
%\newcommand{\aapr}{{\it A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
%\newcommand{\aaps}{{\it A\&AS}}%
          % Astronomy and Astrophysics, Supplement
%\newcommand{\azh}{{\it AZh}}%
          % Astronomicheskii Zhurnal
%\newcommand{\baas}{{\it BAAS}}%
          % Bulletin of the AAS
\newcommand{\caa}{{\it Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{{\it Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
%\newcommand{\icarus}{{\it Icarus}}%
  % Icarus
\newcommand{\jcap}{{\it J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
%\newcommand{\jrasc}{{\it JRASC}}%
          % Journal of the RAS of Canada
%\newcommand{\memras}{{\it MmRAS}}%
          % Memoirs of the RAS
%\newcommand{\mnras}{{\it MNRAS}}%
          % Monthly Notices of the RAS
\newcommand{\na}{{\it New A}}%
  % New Astronomy
\newcommand{\nar}{{\it New A Rev.}}%
  % New Astronomy Review
%\newcommand{\pra}{{\it Phys.~Rev.~A}}%
          % Physical Review A: General Physics
%\newcommand{\prb}{{\it Phys.~Rev.~B}}%
          % Physical Review B: Solid State
%\newcommand{\prc}{{\it Phys.~Rev.~C}}%
          % Physical Review C
%\newcommand{\prd}{{\it Phys.~Rev.~D}}%
          % Physical Review D
%\newcommand{\pre}{{\it Phys.~Rev.~E}}%
          % Physical Review E
%\newcommand{\prl}{{\it Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand{\pasa}{{\it PASA}}%
  % Publications of the Astron. Soc. of Australia
%\newcommand{\pasp}{{\it PASP}}%
          % Publications of the ASP
%\newcommand{\pasj}{{\it PASJ}}%
          % Publications of the ASJ
%\newcommand{\qjras}{{\it QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand{\rmxaa}{{\it Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\skytel}{{\it S\&T}}%
          % Sky and Telescope
%\newcommand{\solphys}{{\it Sol.~Phys.}}%
          % Solar Physics
%\newcommand{\sovast}{{\it Soviet~Ast.}}%
          % Soviet Astronomy
%\newcommand{\ssr}{{\it Space~Sci.~Rev.}}%
          % Space Science Reviews
%\newcommand{\zap}{{\it ZAp}}%
          % Zeitschrift fuer Astrophysik
%\newcommand{\nat}{{\it Nature}}%
          % Nature
%\newcommand{\iaucirc}{{\it IAU~Circ.}}%
          % IAU Cirulars
%\newcommand{\aplett}{{\it Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
%\newcommand{\apspr}{{\it Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
%\newcommand{\bain}{{\it Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
%\newcommand{\fcp}{{\it Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
%\newcommand{\gca}{{\it Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
%\newcommand{\grl}{{\it Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
%\newcommand{\jcp}{{\it J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
%\newcommand{\jgr}{{\it J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
%\newcommand{\jqsrt}{{\it J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand{\memsai}{{\it Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%\newcommand{\nphysa}{{\it Nucl.~Phys.~A}}%
          % Nuclear Physics A
%\newcommand{\physrep}{{\it Phys.~Rep.}}%
          % Physics Reports
%\newcommand{\physscr}{{\it Phys.~Scr}}%
          % Physica Scripta
%\newcommand{\planss}{{\it Planet.~Space~Sci.}}%
          % Planetary Space Science
%\newcommand{\procspie}{{\it Proc.~SPIE}}%
          % Proceedings of the SPIE
